Evaluating Methods for Ground-Truth-Free Foreign Accent Conversion

Foreign accent conversion (FAC) is a special application of voice conversion (VC) which aims to convert the accented speech of a non-native speaker to a native-sounding speech with the same speaker identity. FAC is difficult since the native speech from the desired non-native speaker to be used as the training target is impossible to collect. In this work, we evaluate three recently proposed methods for ground-truth-free FAC, where all of them aim to harness the power of sequence-to-sequence (seq2seq) and non-parallel VC models to properly convert the accent and control the speaker identity. Our experimental evaluation results show that no single method was significantly better than the others in all evaluation axes, which is in contrast to conclusions drawn in previous studies. We also explain the effectiveness of these methods with the training input and output of the seq2seq model and examine the design choice of the non-parallel VC model, and show that intelligibility measures such as word error rates do not correlate well with subjective accentedness. Finally, our implementation is open-sourced to promote reproducible research and help future researchers improve upon the compared systems.

==> figures/materials.tex <==
\begin{figure}[t]
	\centering
	\includegraphics[width=\columnwidth]{figuresmaterials.png}
	\centering
	\captionof{figure}{Common materials for the three evaluated methods in this work. Left: the training data, which is a parallel corpus between the source non-native speaker and a reference native speaker. Right: the non-parallel frame-based VC model, which consists of a pre-trained latent-feature extractor and decoder.}
	\label{fig:materials}
\end{figure}

==> figures/only-methods.tex <==
\begin{figure*}[t]
	\centering
	\includegraphics[width=\textwidth]{only-methods.png}
	\centering
	\captionof{figure}{Illustration of the three evaluated methods (cascade, STG, LSC) in the seq2seq model training phase and the conversion phase. Here all the components from the non-parallel frame-based VC model (marked in blue), including the latent feature extractor and the decoder are trained beforehand and kept fixed in the seq2seq model training phase.}
	\label{fig:methods}
\end{figure*}
